Exploring the high-pressure materials genome

A thorough in situ characterization of materials at extreme conditions is challenging, and computational tools such as crystal structural search methods in combination with ab initio calculations are widely used to guide experiments by predicting the composition, structure, and properties of high-pressure compounds. However, such techniques are usually computationally expensive and not suitable for large-scale combinatorial exploration. On the other hand, data-driven computational approaches using large materials databases are useful for the analysis of energetics and stability of hundreds of thousands of compounds, but their utility for materials discovery is largely limited to idealized conditions of zero temperature and pressure. Here, we present a novel framework combining the two computational approaches, using a simple linear approximation to the enthalpy of a compound in conjunction with ambient-conditions data currently available in high-throughput databases of calculated materials properties. We demonstrate its utility by explaining the occurrence of phases in nature that are not ground states at ambient conditions and estimating the pressures at which such ambient-metastable phases become thermodynamically accessible, as well as guiding the exploration of ambient-immiscible binary systems via sophisticated structural search methods to discover new stable high-pressure phases.

==> NiBi.tex <==
To assess the predictive power of our model for binary compounds, we first investigated the high-pressure phases of the
Ni--Bi intermetallic system. Experimentally, two compounds are known at ambient pressures, \ce{NiBi}~\cite{haegg1929}
and \ce{NiBi3}~\cite{glagoleva1954,ruck2006}. Both phases are superconductors with transition temperatures of
\SI{4.25}{\kelvin} in NiBi~\cite{alekseevskii1952} and \SI{4.06}{\kelvin} in
\ce{NiBi3}~\cite{alekseevskii1948,herrmannsdorfer2011}, respectively. We used structural prototypes from our previous
structural searches of the Fe--Bi and Cu--Bi MHM systems, and substituted the Fe/Cu sites with Ni atoms followed by a
structural relaxation at ambient pressures. The extrapolated enthalpies indicated that high-pressure compounds are
expected to emerge in Ni--Bi at least for the compositions \ce{Ni3Bi} and \ce{NiBi2}. Based on these prediction, we
performed a thorough investigation of the Ni--Bi system by performing MHM runs at pressures of 10 and 50~GPa, which
revealed a plethora of high-pressure phases.


According to our calculations, new high-pressure compounds are predicted at the two experimentally known compositions
\ce{NiBi} and \ce{NiBi3}.  The hexagonal ambient-pressure NiBi phase undergoes a structural transition to the TlI
structure with $Cmcm$ symmetry at pressures above about 20~GPa. Similarly, the $Pnma$ structure of \ce{NiBi3} becomes
thermodynamically unstable above  7.5~GPa, giving way to a $Cmcm$ structure above 62~GPa. Furthermore, we discovered
additional phases at compositions previously unexplored in experiments. Most notably, we found that a \ce{NiBi2} phase
with $C2/m$ symmetry is in fact thermodynamically stable at ambient pressures. At the same composition, a second $C2/m$
emerges above 52~GPa within a very small pressure window of less than 1~GPa, followed by a $I4/mcm$ phase, isostructural
to \ce{FeBi2}. Finally, a \ce{Ni3Bi} compound is predicted at pressures above 25~GPa in the Pmmn structure,
isostructural to XXX.


Fig.~\ref{fig:nibi} shows how the approximate and exact phase diagram of Ni--Bi compared to each other. The qualitative
agreement of the two subplots is almost ideal, and most phases are established to be thermodynamically stable in the
correct pressure sequence within the approximative scheme. The only exceptions are the $Cmcm$ phase at the \ce{NiBi3}
composition and the second $C2/m$ compound at the \ce{NiBi2} composition. The latter phase has only a very small
pressure range of stability, and therefore it is not very surprising that it was missed in the extrapolated phase
diagram. In fact, it might not even be possible to synthesize this phase under practical conditions, similar to the
$Cmcm$ \ce{FeBi3} phase that was initially predicted to be stable within a pressure window of 3~GPa, but not found in
subsequent experiments.


\begin{figure}[tb]
\centering
\subfloat[Exact stability range]{%
  \includegraphics[width=\columnwidth,angle=0]{Figures/NiBi/full_plot/plot_press_conc.pdf}
}\\
\subfloat[Approximated stability range]{%
  \includegraphics[width=\columnwidth,angle=0]{Figures/NiBi/approx_plot_only_stable/plot_press_conc.pdf}
}
\caption{\label{fig:nibi} Exact and approximated stability ranges of Ni--Bi.} 
\end{figure}





==> outline.tex <==
\begin{enumerate}
\item \underline{Introduction and motivation}\\
Two of the most widely-used paradigms of computational materials discovery
are (a) data-driven approaches using large materials databases, and (b)
sophisticated crystal structure prediction (CSP) methods. While (a) are useful
in large-scale analysis of energetics, trends in stability, their utility for
materials discovery at non-ideal conditions is non-existent; intuition derived
from/learning models trained on such ambient-condition data are often not valid
at extreme conditions. For such studies, (b) are applicable, and widely used,
but they are computationally expensive and not viable for extensive
combinatorial exploration.\\

Pressure as a tool to access as-yet undiscovered materials with exotic physics
and chemistries, and extraordinary properties; for example, metallic hydrogen,
Na$_x$Cl$_y$, \ce{NaHe}, \ce{FeBi2}, etc. A lot of merit to extending the
applicability of HT databases to non-ambient pressure conditions, and combining
their quick, exploratory nature with the accuracy, reliability of CSP methods.
Identify chemical spaces with pressure-accessible phases, perform CSP to direct
experimental realization.

With a simple approximation to the enthalpy of a compound, and using
ambient-condition data currently available in large high-throughput databases
such as the OQMD, we:
  \begin{itemize}
  \item gain insights into the effects of pressure on the thermodynamic scale of
  stability/metastability of inorganic compounds
  \item explain the occurrence in nature of phases that are not ground states at
  ambient pressure conditions
  \item estimate the pressures at which ambient-pressure metastable phases
  become thermodynamically stable, and can be accessed experimentally
  \item guide exploration of chemical spaces using pressure as a probe via
  sophisticated CSP methods to discover novel materials
  \end{itemize}

\item \underline{Methods}\\
Briefly describe:
  \begin{itemize}
  \item data available in current high-throughput databases and accessibility
  --- energies, volumes of a large number of experimentally known and
  hypothetical compounds
  \item concept of a convex hull, extension to include volume as an additional
  variable
  \item first-order approximation to the enthalpy of the compound, calculation
  of transition pressures
  \item minima hopping method (MHM) and/or other structure prediction tools
  \end{itemize}
\end{enumerate}


